A New Framework of Software Obfuscation Evaluation Criteria

In the domain of practical software protection against man-at-the-end attacks such as software reverse engineering and tampering, much of the scientific literature is plagued by the use of subpar methods to evaluate the protections' strength and even by the absence of such evaluations. Several criteria have been proposed in the past to assess the strength of protections, such as potency, resilience, stealth, and cost. We analyze their evolving definitions and uses. We formulate a number of critiques, from which we conclude that the existing definitions are unsatisfactory and need to be revised. We present a new framework of software protection evaluation criteria: relevance, effectiveness (or efficacy), robustness, concealment, stubbornness, sensitivity, predictability, and cost.

==> literature.tex <==
\section{Literature study}
\label{sec:literature}
check the A* papers from table 7 in the survey paper: whether or not they have already evaluated all of these criteria

include a table with this data

\begin{table*}[t]
\renewcommand{\arraystretch}{0.9}
\setlength\tabcolsep{2.4pt}
\small %footnotesize
\caption{Goodware papers published in A* venues that De Sutter et al.\ score for how well these implemented their obfuscation evaluation recommendations~\cite{desutter2024evaluation}. Here, these papers are scored for their (implicit or explicit) assessment of all evaluation criteria of our new framework.}\label{tab:scoring_papers}
\centering
\begin{tabular}[t]{ c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c}
    \textbf{Paper}  & \rotatebox{90}{$Re_a$} & \rotatebox{90}{$Re_p$} & \rotatebox{90}{$Re_o$} & \rotatebox{90}{$Re_m$} & \rotatebox{90}{$Re_t$} & \rotatebox{90}{$Re_s$} & \rotatebox{90}{$Re_l$} & \rotatebox{90}{$E_{o,i}$} & \rotatebox{90}{$E_{o,m}$} & \rotatebox{90}{$E_{r,i}$} & \rotatebox{90}{$E_{r,m}$} & \rotatebox{90}{$e_{o,i}$} & \rotatebox{90}{$e_{o,m}$} & \rotatebox{90}{$e_{r,i}$} & \rotatebox{90}{$e_{r,m}$} & \rotatebox{90}{$Ro_o$} & \rotatebox{90}{$Ro_r$} & \rotatebox{90}{$Ro_d$} & \rotatebox{90}{$C_l$} & \rotatebox{90}{$C_s$} & \rotatebox{90}{$C_{si}$} & \rotatebox{90}{$St_o$} & \rotatebox{90}{$St_d$} & \rotatebox{90}{$Se_s$} & \rotatebox{90}{$Se_s$} & \rotatebox{90}{$Se_a$} & \rotatebox{90}{$Se_{pi}$} & \rotatebox{90}{$Se_{pc}$} & \rotatebox{90}{$Se_b$} & \rotatebox{90}{$Se_p$} & \rotatebox{90}{$P_s$} & \rotatebox{90}{$P_s$} & \rotatebox{90}{$P_a$} & \rotatebox{90}{$P_{pi}$} & \rotatebox{90}{$P_{pc}$} & \rotatebox{90}{$P_b$} \\
\hline
%\toprule

\cite{2022_loki_hardening_code_obfuscation_against_automated_attacks} & todo \\
\cite{2022_chosen_instruction_attack_against_commercial_code_virtualization_obfuscators} &todo \\
\cite{2021_search_based_local_black_box_deobfuscation_understand_improve_and_mitigate} & todo \\
\cite{2020_ui_obfuscation_and_its_effects_on_automated_ui_analysis_for_android_apps} &todo \\
\cite{2019_cfhider_control_flow_obfuscation_with_intel_sgx} & todo \\
\cite{2019_asm2vec_boosting_static_representation_robustness_for_binary_clone_search_against_code_obfuscation_and_compiler_optimization} & todo \\
\cite{2019_anything_to_hide_studying_minified_and_obfuscated_code_in_the_web} & todo \\
\cite{2018_software_protection_on_the_go_a_large_scale_empirical_study_on_mobile_app_obfuscation} & todo \\
\cite{2018_protecting_million_user_ios_apps_with_obfuscation_motivations_pitfalls_and_experience} & todo \\
\cite{2018_hybrid_obfuscation_to_protect_against_disclosure_attacks_on_embedded_microprocessors} & todo \\
\cite{2017_syntia_synthesizing_the_semantics_of_obfuscated_code} & todo \\
\cite{liu2017stochastic} & todo \\
\cite{2017_semantics_based_obfuscation_resilient_binary_code_similarity_comparison_with_applications_to_software_and_algorithm_plagiarism_detection} & todo \\
\cite{2017_recovering_clear_natural_identifiers_from_obfuscated_js_names} &todo \\
\cite{2017_predicting_the_resilience_of_obfuscated_code_against_symbolic_execution_attacks_via_machine_learning} & todo \\
\cite{2016_reliable_third_party_library_detection_in_android_and_its_security_applications} & todo \\
\cite{2010_mimimorphism_a_new_approach_to_binary_code_obfuscation} & todo \\
\cite{2007_binary_obfuscation_using_signals} & todo \\
\cite{2004_static_disassembly_of_obfuscated_binaries} &  todo \\
\cite{Linn2003} & todo \\
\cite{collberg1998manufacturing} & todo \\

\hline
%\bottomrule
     \end{tabular}
 \end{table*}
